3PC: Three Point Compressors for Communication-Efficient Distributed Training and a Better Theory for Lazy Aggregation

We propose and study a new class of gradient communication mechanisms for communication-efficient training -- three point compressors (3PC) -- as well as efficient distributed nonconvex optimization algorithms that can take advantage of them. Unlike most established approaches, which rely on a static compressor choice (e.g., Top-$K$), our class allows the compressors to {\em evolve} throughout the training process, with the aim of improving the theoretical communication complexity and practical efficiency of the underlying methods. We show that our general approach can recover the recently proposed state-of-the-art error feedback mechanism EF21 (Richt\'arik et al., 2021) and its theoretical properties as a special case, but also leads to a number of new efficient methods. Notably, our approach allows us to improve upon the state of the art in the algorithmic and theoretical foundations of the {\em lazy aggregation} literature (Chen et al., 2018). As a by-product that may be of independent interest, we provide a new and fundamental link between the lazy aggregation and error feedback literature. A special feature of our work is that we do not require the compressors to be unbiased.

==> preamble.tex <==


\usepackage{euscript}	 %  
\usepackage{makecell}

\usepackage{times}
\RequirePackage{fix-cm}
\usepackage{cmap}					%   PDF

\usepackage{comment}
\usepackage{xr}

%\usepackage[noend]{algpseudocode}

%\usepackage{extsizes} %   14- 
%\usepackage{geometry} %    
\usepackage{url}
\usepackage{csquotes} %   
\usepackage{siunitx}
\usepackage{float}
\restylefloat{table}
\usepackage{array}

\usepackage{nicefrac}

%\usepackage{undertilde}

\usepackage{setspace} % 
%\onehalfspacing %  1.5
%\doublespacing %  2
%\singlespacing %  1
\usepackage[export]{adjustbox}
\usepackage{lastpage} % ,     .
\usepackage{soulutf8} %  
\usepackage{icomma} % "" : $0,2$ --- , $0, 2$ --- 

%\newenvironment{solution}
%{\renewcommand\qedsymbol{$\blacksquare$}\begin{proof}[Solution]}{\end{proof}}

\usepackage[flushleft]{threeparttable} % http://ctan.org/pkg/threeparttable

\usepackage{etoolbox}
%\usepackage{mathtools}
\usepackage{etextools}
\usepackage{ifthen}
\usepackage{caption}
%\usepackage{subcaption}
\usepackage{amsmath,amssymb, amsthm}
%\usepackage{charter}
%\usepackage{calc}

\usepackage{calligra}
\usepackage{amsfonts}
\usepackage{layout}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{hyperref}%[backref=true]
% \usepackage[colorlinks,linkcolor=magenta,citecolor=blue, pagebackref=true,backref=true]{hyperref}
\usepackage{cleveref}
\usepackage{lipsum}
%\usepackage{mathtools}
%\mathtoolsset{showonlyrefs=true}
%\usepackage{mathrsfs}
\usepackage{url}
\usepackage{color}
\usepackage{url}
\usepackage{color}
\usepackage{setspace}

\usepackage{multicol} %  
\usepackage{filecontents}
%nwork with tables
\usepackage{array,tabularx,tabulary,booktabs} %    
%\usepackage{longtable}  %  
\usepackage{multirow} %    
\usepackage{graphicx}
%\usepackage{subfig}
\usepackage{fancyhdr}
%\usepackage{theoremref}

\usepackage{pifont}%for defining \xmark


%%%%%%%%%%%%%%
%NEW COMMANDS   %%%
%%%%%%%%%%%%%%

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\sign}{sign}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}

\newcommand{\z}{\zeta}
\newcommand{\lt}{\left}
\newcommand{\rt}{\right}
\newcommand{\al}{\alpha}
\newcommand{\p}{\partial}
\newcommand{\D}{\Delta}
\newcommand{\nfr}{\nicefrac}
\newcommand{\fr}{\frac}
\newcommand{\dfr}{\dfrac}
\newcommand{\mbf}{\mathbf}
\newcommand{\mds}{\mathds}
\newcommand{\bb}{\mathbb}
\newcommand{\wt}{\widetilde}
\newcommand{\wS}{\wt{S}}
\newcommand{\wA}{\wt{A}}
\newcommand{\tA}{\tilde{A}}
\newcommand{\sigmt}{\sigma^{t}}
\newcommand{\sigmtpo}{\sigma^{t+1}}
\newcommand{\tB}{\tilde{B}}
\newcommand{\tC}{\tilde{C}}
\newcommand{\ttheta}{\tilde{\theta}}
\newcommand{\wAi}{\wt{A}_i}
\newcommand{\wL}{\wt{L}}
\newcommand{\wai}{\wt{a}_i}
\newcommand{\wa}{\wt{a}}
\newcommand{\wc}{\wt{c}}
\newcommand{\wtd}{\wt{d}}
\newcommand{\wsigma}{\wt{\sigma}}
\newcommand{\wLi}{\wt{L}_i}
\newcommand{\wwL}{\wt{\wt{L}}}
\newcommand{\wB}{\wt{B}}
\newcommand{\wC}{\wt{C}}
\newcommand{\ws}{\wt{s}}
\newcommand{\wg}{\wt{g}}
\newcommand{\wgt}{\wt{g}^t}
\newcommand{\wgtpo}{\wt{g}^{t+1}}
\newcommand{\wgit}{\wg_i^t}
\newcommand{\wgitpo}{\wg_i^{t+1}}
\newcommand{\wgix}{\wg_i(x)}
\newcommand{\wgiy}{\wg_i(y)}
\newcommand{\wgik}{\wg_i(x^k)}
\newcommand{\wgikpo}{\wg_i(x^{k+1})}
\newcommand{\wgu}{\wt{g}^u}
\newcommand{\wG}{\wt{G}}
\newcommand{\hL}{\hat{L}}
\newcommand{\hG}{\hat{G}}
\newcommand{\hAi}{\hat{A}_i}
\newcommand{\hA}{\hat{A}}
\newcommand{\hB}{\hat{B}}

\newcommand{\hC}{\hat{C}}
\newcommand{\hD}{\hat{D}}
\newcommand{\pA}{A^{\prime}}
\newcommand{\pB}{B^{\prime}}
\newcommand{\pC}{C^{\prime}}
\newcommand{\wpA}{\wA^{\prime}}
\newcommand{\wpB}{\wB^{\prime}}
\newcommand{\wpC}{\wC^{\prime}}
\newcommand{\ppA}{A^{\prime \prime}}
\newcommand{\ppB}{B^{\prime \prime}}
\newcommand{\ppC}{C^{\prime \prime}}


\newcommand{\hg}{\hat{g}}
\newcommand{\hf}{\hat{f}}
\newcommand{\hgi}{\hat{g}_i}
\newcommand{\hgix}{\hat{g}_i(x)}
\newcommand{\hgiy}{\hat{g}_i(y)}
\newcommand{\hgik}{\hat{g}_i(x^k)}
\newcommand{\hgikpo}{\hat{g}_i(x^{k+1})}
\newcommand{\hgit}{\hat{g}_i(x^t)}
\newcommand{\hgitpo}{\hat{g}_i(x^{t+1})}
\newcommand{\hgu}{\hat{g}^u}
\newcommand{\hs}{\hat{s}}


\newcommand{\eik}{e_i^t}
\newcommand{\gik}{g_i^t}
\newcommand{\gikpo}{g_i^{t+1}}
\newcommand{\eikpo}{e_i^{t+1}}
\newcommand{\vik}{v_i^t}
\newcommand{\vikpo}{v_i^{t+1}}

\newcommand{\eit}{e_i^t}
\newcommand{\eitpo}{e_i^{t+1}}
%\newcommand{\vit}{v_i^t}
%\newcommand{\vitpo}{v_i^{t+1}}

\newcommand{\wcC}{\wt{\cC}}
\newcommand{\La}{\Lambda}
\newcommand{\lam}{\lambda}
\newcommand{\lami}{\lam_i}
\newcommand{\opn}{\operatorname}
\newcommand{\vp}{\varphi}
\newcommand{\bM}{\mbf M}
\newcommand{\bG}{\mbf G}
\newcommand{\bI}{\mbf I}
\newcommand{\bD}{\mbf D}
\newcommand{\bA}{\mbf A}
\newcommand{\bC}{\mbf C}
\newcommand{\bP}{\mbf P}
\newcommand{\bB}{\bb B}
\newcommand{\bU}{\bb U}
\newcommand{\bLa}{\mbf {\La}}
\newcommand{\R}{\bb R}
\newcommand{\bE}{\mbf E}
\newcommand{\hS}{\hat{S}}
\newcommand{\eps}{{\varepsilon}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\stepsize}{\eta}

\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\lin}[1]{\left\langle #1\right\rangle} % product

\newcommand{\cE}{{\cal E}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cM}{{\cal M}}

\newcommand{\wcL}{\wt{\mathcal{L}}}
\newcommand{\cCw}{\cC_{\omega}}
\newcommand{\cCd}{\cC_{\delta}}
\newcommand{\Ctk}[1]{\cC_{Tk}\rb{#1}}
\newcommand{\gixk}{g_{i}(x_k)}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\mM}{\mathbf{M}}
\newcommand{\mN}{\mathbf{N}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\mI}{\mathbf{I}}
\newcommand{\mL}{\mathbf{L}}
\newcommand{\mD}{\mathbf{D}}
\newcommand{\bx}{\bar{x}}
\newcommand{\by}{\bar{y}}
\newcommand{\barA}{\overline{A}}
\newcommand{\barB}{\overline{B}}
\newcommand{\barL}{\overline{L}}
\newcommand{\barC}{\overline{C}}
\newcommand{\barD}{\overline{D}}
\newcommand{\bara}{\overline{a}}
\newcommand{\eqtext}[1]{\ensuremath{\stackrel{\text{#1}}{=}}}
\newcommand{\letext}[1]{\ensuremath{\stackrel{\text{#1}}{\le}}}
\newcommand{\getext}[1]{\ensuremath{\stackrel{\text{#1}}{\ge}}}
\newcommand{\succtext}[1]{\ensuremath{\stackrel{\text{#1}}{\succ}}}
\newcommand{\preceqtext}[1]{\ensuremath{\stackrel{\text{#1}}{\preceq}}}
\newcommand{\onenorm}[1]{\left\| #1 \right\|_1}      % norm 
\newcommand{\twonorm}[1]{\left\| #1 \right\|_2}      % norm 
\newcommand{\threenorm}[1]{\left\| #1 \right\|_3}      % norm 
\newcommand{\gnorm}[1]{\left\| #1 \right\|^{1 + \gamma }}      % norm 
\newcommand{\sqnorm}[1]{\left\| #1 \right\|^{2}}
\newcommand{\anorm}[1]{\left\| #1 \right\|^{\al}}      % norm 
\newcommand{\bnorm}[1]{\left\| #1 \right\|^{\beta}}      % norm 
\newcommand{\ahnorm}[1]{\left\| #1 \right\|^{\al/2}}      % norm 
\newcommand{\bbone}[1]{\mathbb{1}}      % norm 
\newcommand{\g}{\gamma}

\newcommand{\nf}[1]{\nabla f\rb{#1}}      % norm 

\newcommand{\hotidea}{{\color{red}\bf HOT IDEA: }}
\newcommand{\done}{{\color{blue}\bf DONE: }}


\newcommand{\del}[1]{}

\newcommand{\finf}{f^\mathrm{inf}}
\newcommand{\fiinf}{f_i^\mathrm{inf}}

\let\la=\langle
\let\ra=\rangle

\def\<{\left\langle}
\def\>{\right\rangle}
% \def\[{\left[}
%\def\]{\right]}
\def\({\left(}
\def\){\right)}

%\newcommand{\st}{\;:\;}
\newcommand{\ve}[2]{\langle #1 ,  #2 \rangle}

%\newcommand{\eqdef}{\stackrel{\text{def}}{=}}
\newcommand{\eqdef}{:=}

\newcommand{\ii}{{}^{(i)}}


\newcommand{\Prob}{\mathbf{Prob}}
\newcommand{\E}{\mathbf{E}}

%\usepackage{bbm}
%\usepackage{dsfont}

\newcommand{\vc}[2]{#1^{(#2)}}
\newcommand{\nc}[2]{{\color{red}\|#1\|_{(#2)}}}
\newcommand{\ncs}[2]{\|#1\|^2_{(#2)}}
\newcommand{\ncc}[2]{{\color{red}\|#1\|^*_{(#2)}}}
\newcommand{\ls}[1]{{\color{red} \mathcal S(#1)}}
\newcommand{\Rw}[2]{\mathcal R_{#1}(#2)}
\newcommand{\Rws}[2]{\mathcal R^2_{#1}(#2)}

\newcommand{\nbp}[2]{\|#1\|_{(#2)}}   % norm block primal
\newcommand{\nbd}[2]{\|#1\|_{(#2)}^*} % norm block dual

\newcommand{\lf}{\mathcal L}
\newcommand{\U}{U}
\newcommand{\N}{N}

\newcommand{\mLi}{{\color{red}m^{(i)}}}
\newcommand{\gLi}{{\color{red}f{(i)}}}
%\newcommand{\TLi}{{\color{red}T_L^{(i)}}}
\newcommand{\TLi}[1]{{\color{blue}T^{(#1)}}}

\newcommand{\Lip}{L}

\newcommand{\Rc}[1]{{\color{red}  \mathbf{RC}_{(#1)}}}
\newcommand{\NRCDM}{{\color{red}NRCDM}\  }
\newcommand{\nnz}[1]{{\color{red}\|#1\|_0}}
% sets
\DeclareMathOperator{\card}{card}       % cardinality of a set
\DeclareMathOperator{\diam}{diam}       % diameter of a set
\DeclareMathOperator{\MVEE}{MVEE}       % minim volume enclosing ellipsoid of a set
\DeclareMathOperator{\vol}{vol}         % volume of a set

% statistical
% \DeclareMathOperator{\Exp}{{\rm E}}           % expectation
%\newcommand{\Exp}[1]{{\rm E}\left[#1\right]}
\newcommand{\Exp}[1]{{\bb E}\left[#1\right]}
\newcommand{\Expu}[2]{{\bb E}_{#1}\left[#2\right]}

\DeclareMathOperator{\Cov}{Cov}         % covariance
\DeclareMathOperator{\Var}{Var}         % variance
\DeclareMathOperator{\Corr}{Corr}       % correlation

% functions and operators
\DeclareMathOperator{\signum}{sign}     % signum/sign of a scalar
\DeclareMathOperator{\dom}{dom}         % domain
\DeclareMathOperator{\epi}{epi}         % epigraph
\DeclareMathOperator{\Ker}{null}        % nullspace/kernel
\DeclareMathOperator{\nullspace}{null}  % nullpsace
\DeclareMathOperator{\range}{range}     % range
\DeclareMathOperator{\Image}{Im}        % image

% topology
\DeclareMathOperator{\interior}{int}    % interior
\DeclareMathOperator{\ri}{rint}         % relative interior
\DeclareMathOperator{\rint}{rint}       % relative interior
\DeclareMathOperator{\bdry}{bdry}       % boundary
\DeclareMathOperator{\cl}{cl}           % closure

% vectors, matrices
\DeclareMathOperator{\linspan}{span}
\DeclareMathOperator{\linspace}{linspace}
\DeclareMathOperator{\cone}{cone}

%\DeclareMathOperator{\tr}{tr}           % trace
\DeclareMathOperator{\rank}{rank}       % rank
\DeclareMathOperator{\conv}{conv}       % convex hull
\DeclareMathOperator{\Diag}{Diag}       % Diag(v) = diagonal matrix with v_i on the diagonal
\DeclareMathOperator{\diag}{diag}       % diag(D) = the diagonal vector of matrix D

\DeclareMathOperator{\Arg}{Arg}         % Argument

%\renewcommand{\qedsymbol}{\ding{114}}

\newcommand{\lamax}[1]{\lam_{\max}\left(#1\right)}
\newcommand{\lamin}[1]{\lam_{\min}\left(#1\right)}
\newcommand{\rb}[1]{\left(#1\right)}
\renewcommand{\sb}[1]{\left[#1\right]}
\newcommand{\cb}[1]{\lt\{#1\rt\}}

\newcommand {\rbl}[1]{(#1)} %round braces without left - right alignment
\renewcommand{\nf}[1]{\nabla f\rbl{#1}}
\newcommand{\nfi}[1]{\nabla f_i\rbl{#1}}
\newcommand{\nfj}[1]{\nabla f_j\rbl{#1}}

\newcommand{\vtp}{v^{t-1}}
\newcommand{\vt}{v^{t}}
\newcommand{\vtpo}{v^{t+1}}

\newcommand{\yijt}{y_{ij}^t}
\newcommand{\yilt}{y_{il}^t}
\newcommand{\yijtpo}{y_{ij}^{t+1}}
\newcommand{\yiltpo}{y_{il}^{t+1}}
\newcommand{\vitp}{v_i^{t-1}}
\newcommand{\vit}{v_i^{t}}
\newcommand{\vitpo}{v_i^{t+1}}

%\newcommand{\dgit}{\Delta g_i^{t}}
%\newcommand{\dgitpo}{\Delta g_i^{t+1}}
%\newcommand{\dgitpm}{\Delta g_i^{t-1}}
\newcommand{\git}{g_i^t}
\newcommand{\gitpo}{g_i^{t+1}}
\newcommand{\gitpm}{g_i^{t-1}}
\newcommand{\dgit}{\vit}
\newcommand{\dgitpo}{\vitpo}
\newcommand{\dgitpm}{\gitpm}

\newcommand{\xk}{x^{k}}
\newcommand{\xt}{x^{t}}
\newcommand{\yt}{y^{t}}
\newcommand{\xtpo}{x^{t+1}}
\newcommand{\ytpo}{y^{t+1}}
\newcommand{\xitpo}{\xi^{t+1}}
\newcommand{\xit}{\xi^{t}}
%\newcommand{\xtp}{x^{t-1}}

%\newcommand{\omtpo}{\omega^{t+1}}
%\newcommand{\omt}{\omega^{t}}
%\newcommand{\omi}{\omega_i}
%\newcommand{\om}{\omega}
\newcommand{\omi}{w_i}
\newcommand{\om}{w}

\newcommand{\omtpo}{w^{t+1}}
\newcommand{\omt}{w^{t}}

\newcommand{\xkpo}{x^{k+1}}
\newcommand{\fxk}{f(\xk)}
\newcommand{\gxk}{g(\xk)}
\newcommand{\fxkpo}{f(\xkpo)}
\newcommand{\dz}{\delta_0}
\newcommand{\xs}{x^{\star}}
\newcommand{\nfxk}{\nf{\xk}}
\newcommand{\nfxkpo}{\nf{x^{k+1}}}
\newcommand{\nfxt}{\nf{\xt}}
\newcommand{\nfxtpo}{\nf{\xtpo}}
\newcommand{\nfomt}{\nf{\omt}}
\newcommand{\nfomtpo}{\nf{\omtpo}}
\newcommand{\nfxs}{\nf{\xs}}
\newcommand{\nfx}{\nf{x}}
\newcommand{\nfy}{\nf{y}}
\newcommand{\nfxijk}{\nabla f_{\xi_{ij}^k} (x^k)}
\newcommand{\nfxijkpo}{\nabla f_{\xi_{ij}^k}(x^{k+1})}
\newcommand{\nfixk}{\nfi{\xk}}
\newcommand{\nfixt}{\nfi{\xt}}
\newcommand{\nfix}{\nfi{x}}
\newcommand{\nfiy}{\nfi{y}}
\newcommand{\nfij}[1]{\nabla f_{ij}\rbl{#1}}
\newcommand{\nfil}[1]{\nabla f_{il}\rbl{#1}}
\newcommand{\nfijxt}{\nfij{\xt}}
\newcommand{\nfijxtpo}{\nfij{\xtpo}}
\newcommand{\nfjxtpo}{\nfj{\xtpo}}
\newcommand{\nfjomtpo}{\nfj{\omtpo}}
\newcommand{\nfijomiit}{\nfij{\omiit}}
\newcommand{\nfiomiit}{\nfi{\omiit}}
\newcommand{\nfijomiitpo}{\nfij{\omiitpo}}
\newcommand{\nfilomiit}{\nfil{\omiit}}
\newcommand{\nfilomiitpo}{\nfil{\omiitpo}}
\newcommand{\nfilxt}{\nfil{\xt}}
\newcommand{\nfilxtpo}{\nfil{\xtpo}}
\newcommand{\nfijx}{\nabla f_{ij}(x)}
\newcommand{\nfijy}{\nabla f_{ij}(y)}
\newcommand{\dgt}{\Delta g^{t}}
\newcommand{\dgtpo}{\Delta g^{t+1}}
\newcommand{\gt}{ g^{t}}
\newcommand{\gtpo}{ g^{t+1}}

%\newcommand{\omiitpo}{\omega_i^{t+1}}
%\newcommand{\omijt}{\omega_{ij}^{t}}
%\newcommand{\omilt}{\omega_{il}^{t}}
%\newcommand{\omijtpo}{\omega_{ij}^{t+1}}
%\newcommand{\omiltpo}{\omega_{il}^{t+1}}
%\newcommand{\omiit}{\omega_i^{t}}

\newcommand{\omiitpo}{w_i^{t+1}}
\newcommand{\omijt}{w_{ij}^{t}}
\newcommand{\omilt}{w_{il}^{t}}
\newcommand{\omijtpo}{w_{ij}^{t+1}}
\newcommand{\omiltpo}{w_{il}^{t+1}}
\newcommand{\omiit}{w_i^{t}}


\newcommand{\nfiomtpo}{\nfi{\omitpo}}
\newcommand{\nfitpoxtpo}{\nabla f_{i_{t+1}}(x^{t+1})}

%\newcommand{\nfix}{\nfi{x}}

\newcommand{\nfixs}{\nfi{\xs}}
\newcommand{\nfjxk}{\nfj{\xk}}
\newcommand{\nfjxs}{\nfj{\xs}}
\newcommand{\nfixkpo}{\nfi{x^{k+1}}}
\newcommand{\nfixtpo}{\nfi{x^{t+1}}}
\newcommand{\nfitxt}{\nabla f_{i_{t}}(x^{t})}
\newcommand{\nfitomt}{\nabla f_{i_{t}}(\omt)}
%\newcommand{\nfitpoxtpo}{\nabla f_{i_{t+1}}(x^{t+1})}
\newcommand{\nfitpoomtpo}{\nabla f_{i_{t+1}}(\omtpo)}

\newcommand{\nfjxkpo}{\nfj{x^{k+1}}}
\newcommand{\hik}{h^{k}_{i}}
\newcommand{\ali}{\al_{i}}
\newcommand{\mik}{m^{k}_{i}}
\newcommand{\hikpo}{h^{k+1}_{i}}
\newcommand{\hk}{h^{k}}
\newcommand{\nmo}{\fr{1}{n}}
\newcommand{\nmt}{\fr{1}{n^2}}
\newcommand{\tnmo}{\fr{2}{n}}
\newcommand{\tnmt}{\fr{2}{n^2}}
\newcommand{\ub}{\underbrace}





\newcommand {\maxin}{\max_{i=1,\dots, n}}
\newcommand {\maxi}{\max_{i}}
\newcommand {\minin}{\min_{i=1,\dots, n}}
\newcommand {\mini}{\min_{i}}
\newcommand {\sumin}{\sum_{i=1}^{n}}
\newcommand {\sumtt}{\sum_{t=0}^{T}}
\newcommand {\sumlmi}{\fr{1}{m_i}\sum_{l=1}^{m_i}}
\newcommand {\suminn}{\fr{1}{n}\sum_{i=1}^{n}}
\newcommand {\sumjm}{\sum_{j=1}^{m}}
\newcommand {\sumjmi}{\sum_{j=1}^{m_i}}
\newcommand {\sumjmm}{\fr{1}{m}\sum_{j=1}^{m}}
\newcommand {\sumjnn}{\fr{1}{n}\sum_{j=1}^{n}}
\newcommand {\sumjmmi}{\fr{1}{m_i}\sum_{j=1}^{m_i}}
\newcommand {\sumjn}{\sum_{j=1}^{n}}
\newcommand {\wik}{w_{i}^{k}}
\newcommand {\wjk}{w_{j}^{k}}
\newcommand {\wk}{w^{k}}
\newcommand {\wikpo}{w_{i}^{k+1}}
\newcommand {\wjkpo}{w_{j}^{k+1}}
%\newcommand {\sumin}{\sum_{i=1}^{n}}
\newcommand {\sumid}{\sum_{i=1}^{d}}
\newcommand {\ghx}{\hat{g}(x)}
\newcommand {\gh}{\hat{g}}
\newcommand {\gih}{\hat_i}
\newcommand {\gihx}{\hat{g_i}(x)}
%\newcommand {\sumjn}{\sum_{j=1}^{n}}
\newcommand{\cmark}{\textcolor{green}{\ding{51}}}%
\newcommand{\xmark}{\textcolor{red}{\ding{55}}}%

\DeclareMathOperator{\tr}{Tr}
% \renewcommand{\tr}[1]{\tr\left(#1\right)}

%\newtheorem{example}{Example}
%\newtheorem{assumption}{Assumption}
%\newtheorem{lemma}{Lemma}

%\usepackage[noend]{algpseudocode}
%\usepackage{verbatim}
%\usepackage[ruled,vlined]{algorithm2e}
%\usepackage{algorithm}
%\usepackage{algpseudocode}

%\newtheorem{theorem}{Theorem}
%\newtheorem{proposition}{Proposition}
%
%\theoremstyle{plain}
%
%\newtheorem{prop}[theorem]{Proposition}
%\newtheorem{corollary}{Corollary}
%\newtheorem{lem}[theorem]{Lemma}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{remark}{Remark}
%
%
%\newtheorem{exercise}[theorem]{Exercise}
%
%\newtheorem{rem}[theorem]{Remark}
%\newtheorem{que}[theorem]{Question}
%\newtheorem{definition}{Definition}


%zerosarah paper symbols

\newcommand*{\qedb}{\hfill\ensuremath{\square}}   % or \blacksquare
\newcommand{\topic}[1]{\vspace{2mm}\noindent{{\bf #1:}}}
\newcommand{\head}[1]{\noindent{{\bf #1:}}}
%\newcommand{\red}[1]{\textcolor{red}{#1}}
%\newcommand{\blue}[1]{\textcolor{blue}{#1}}

\newcommand{\zerosarah}{{\sf ZeroSARAH}\xspace}



\usepackage{xspace}

%TODO: copypaste to the main preamble file
\newcommand{\bit}{b_i^t}
\newcommand{\bt}{b^t}
\newcommand{\Lpm}{L_{\pm}}

%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{tcolorbox}
\usepackage{pifont}
\definecolor{mydarkgreen}{RGB}{39,130,67}
\definecolor{mydarkred}{RGB}{192,47,25}
\definecolor{mydarkblue}{RGB}{39,47,180}
\newcommand{\green}{\color{mydarkgreen}}
\newcommand{\red}{\color{mydarkred}}
\newcommand{\blue}{\color{mydarkblue}}
%\newcommand{\cmark}{\green\ding{51}}%
%\newcommand{\xmark}{\red\ding{55}}%

\newcommand{\algname}[1]{{\sf \footnotesize \green #1}\xspace}


\newcommand{\squeeze}{\textstyle}
\newcommand{\thetaNEW}{{\red A}}
\newcommand{\betaNEW}{{\red B}}
\newcommand{\alphaNEW}{{\green\alpha}}
\newcommand{\lambdaNEW}{\alpha}

